Equivariant Segre and Verlinde invariants for Quot schemes

The problem of studying the two seemingly unrelated sets of invariants forming the Segre and the Verlinde series has gone through multiple different adaptations including a version for the virtual geometries of Quot schemes on surfaces and Calabi-Yau fourfolds. Our work is the first one to address the equivariant setting for both $\mathbb{C}^2$ and $\mathbb{C}^4$ by examining higher degree contributions which have no compact analogue. (1) For $\mathbb{C}^2$, we work mostly with virtual geometries of Quot schemes. After connecting the equivariant series in degree zero to the existing results of the first author for compact surfaces, we extend the Segre-Verlinde correspondence to all degrees and to the reduced virtual classes. Apart from it, we conjecture an equivariant symmetry between two different Segre series building again on previous work. (2) For $\mathbb{C}^4$, we give further motivation for the definition of the Verlinde series. Based on empirical data and additional structural results, we conjecture the equivariant Segre-Verlinde correspondence and the Segre-Segre symmetry analogous to the one for $\mathbb{C}^2$.

==> temp.tex <==


